Content-centric Routing in Wi-Fi Direct Multi-group Networks

The added value of Device-to-Device (D2D) communication amounts to an efficient content discovery mechanism that enables users to steer their requests toward the node most likely to satisfy them. In this paper, we address the implementation of content-centric routing in a D2D architecture for Android devices based on WiFi Direct, a protocol recently standardised by the Wi-Fi Alliance. After discussing the creation of multiple D2D groups, we introduce novel paradigms featuring intra- and inter-group bidirectional communication. We then present the primitives involved in content advertising and requesting among members of the multi-group network. Finally, we evaluate the performance of our architecture in a real testbed involving Android devices in different group configurations. We also compare the results against the ones achievable exploiting Bluetooth technologies.

==> biblio.tex <==
\begin{thebibliography}{99}

\bibitem{TomsHardware2012} Tom's Hardware, Report over 5 billion
wireless chips shipping in 2013, \url{http://www.tomshardware.com}, 2013.

\bibitem{Alljoyn2013} Qualcomm, AllJoyn, \url{http://www.alljoyn.org}, 2013.

\bibitem{Intel2013} INTEL Common Connectivity Framework, 
  \url{http://intel-common-connectivity-framework.software.informer.com/}, 2013.

\bibitem{Wi-FiAlliance2013} Wi-Fi Alliance,
\url{http://www.wi-fi.org/discover-and-learn/wi-fi-certified-passpoint\%E2\%84\%A2}, 2013.


\bibitem{Sachs2010} 
J. Sachs, M.  Olsson,  ``Access Network Discovery and Selection in the Evolved 3GPP
Multi-access System Architecture,'' {\em European Transactions in Telecommunications}, No.\,6, Vol.\,21, Oct.\,2010.

\bibitem{duong}
T.N. Duong, N.T. Dinh, Y. Kim, ``Content sharing using P2PSIP Protocol
in Wi-Fi Direct Networks,'' 
{\em International Conference on Communications and Electronics (ICCE),} Hue, Vietnam Aug.\,2012.

\bibitem{Lim2013}
Keun Woo Lim and Woo Sung Jung and Kim, H. and Han, J. and Young Bae Ko, ``Enhanced power management for Wi-Fi Direct,'' {\em Wireless Communications and Networking Conference (WCNC),} Apr.\,2013.

\bibitem{Conti2013}
M. Conti, F. Delmastro, G. Minutiello, R. Paris, ``Experimenting
opportunistic networks with WiFi Direct,'' {\em IFIP Wireless Days (WD),} Valencia, Spain, Nov.\,2013.

\bibitem{camps-mur} 
D. Camps-Mur, A. Garcia-Saavedra, P. Serrano, ``Device-to-device communications with Wi-Fi Direct: overview and experimentation,'' {\em IEEE Wireless Communications,} Vol.\,20, pp.\,96--104, June 2013.

\bibitem{camps-mur2011} 
D. Camps-Mur, X. Perez-Costa, S. Sallent-Ribes, ``Designing energy efficient access points with Wi-Fi Direct,'' {\em Computer Networks,} Vol.\,55, pp.\,2838--2855, Sep.\,2011.

\bibitem{lombera} 
I.M. Lombera, L.E. Moser, P.M. Melliar-Smith, Y.T. Chuang, ``Peer
management for iTrust over Wi-Fi Direct,'' {\em Wireless Personal Multimedia Communications (WPMC),} Atlantic City, NJ, June 2013.

\bibitem{Mancuso} A. Asadi, V. Mancuso, ``WiFi Direct and LTE D2D in
  action,'' {\em IFIP Wireless Days (WD),} Valencia, Spain, Nov.\,2013.

\bibitem{noi} 
\end{thebibliography}


==> test.tex <==
\section{Performance evaluation}


\subsection{Methology}
\color{red}PLEASE DESCRIBE HERE THE METHODOLOGY: configuration, measurement tools, number of runs, etc., in order to allow a reader to reproduce the experimentation
\color{black}

\subsection{Tunneling mechanism}

\color{red}PLEASE DESCRIBE HERE THE ACHIEVABLE PERFORMANCE . SHOW FIGURES AND 

\color{black}


\subsection{Service discovery and provisioning}
\color{red}PLEASE DESCRIBE HERE THE ACHIEVABLE PERFORMANCE . SHOW FIGURES AND 

\color{black}



 
